SparseCam4D: Spatio-Temporally Consistent 4D Reconstruction from Sparse Cameras

High-quality 4D reconstruction enables photorealistic and immersive rendering of the dynamic real world. However, unlike static scenes that can be fully captured with a single camera, high-quality dynamic scenes typically require dense arrays of tens or even hundreds of synchronized cameras. Dependence on such costly lab setups severely limits practical scalability. To this end, we propose a sparse-camera dynamic reconstruction framework that exploits abundant yet inconsistent generative observations. Our key innovation is the Spatio-Temporal Distortion Field, which provides a unified mechanism for modeling inconsistencies in generative observations across both spatial and temporal dimensions. Building on this, we develop a complete pipeline that enables 4D reconstruction from sparse and uncalibrated camera inputs. We evaluate our method on multi-camera dynamic scene benchmarks, achieving spatio-temporally consistent high-fidelity renderings and significantly outperforming existing approaches. Project page available at https://inspatio.github.io/sparse-cam4d/

==> fig/ablation-rcm.tex <==
\centering
\begin{minipage}{0.99\linewidth} % 图片区域    
    \centering        
    \includegraphics[width=\linewidth]{files/ablation-rcm.pdf}  
\end{minipage}
\label{fig:ablation-rcm}


==> fig/ablation.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.96\linewidth} % 图片区域    
        \centering        
        \includegraphics[width=\linewidth]{files/ablation3_train.pdf}  
    \end{minipage}
    \vspace{-3mm}
    \caption{ % caption
      \textbf{Qualitative ablation results.} 
         Rendering results (a) and space-time slices (b), constructed by concatenating the red pixel locations across all time steps, demonstrate that direct reconstruction from diffusion observations results in severe blur and temporal instability.
        }    
\label{fig:ablation}
\vspace{-3mm}
\end{figure}

==> tab/ablation-rcm.tex <==
\setlength\tabcolsep{3.5pt}
\resizebox{0.48\linewidth}{!}{%
\begin{tabular}{lccc}
    \toprule[1.5pt]
    & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
    \midrule
    ViewCrafter      & 21.42 & 0.775 & 0.302 \\
    Ours-ViewCrafter & 23.93 & 0.832 & 0.232 \\
    ReCamMaster      & 21.97 & 0.756 & 0.315 \\
    Ours-ReCamMaster & 23.61 & 0.806 & 0.247 \\
    \bottomrule[1.5pt]
\end{tabular}
}

==> tab/ablation2.tex <==
\begin{table}[htbp]    
    \caption{\textbf{Ablation studies.} We random select one representative scene from Technicolor~\citep{sabater2017dataset} and Nvidia Dynamic Scenes~\citep{yoon2020novel} Datasets to ablate our framework.}
    \centering
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}[t]{l|ccc|ccc}    
        \toprule[2pt]
        \multirow{2}{*}{Setting}        
        &\multicolumn{3}{c|}{\textbf{Train}}%~\citep{sabater2017dataset}}
        &\multicolumn{3}{c}{\textbf{Jumping}}%~\citep{yoon2020novel}}\\
        \\
        &\text{PSNR}$\uparrow$&\text{SSIM}$\uparrow$&\text{LPIPS}$\downarrow$
        &\text{PSNR}$\uparrow$&\text{SSIM}$\uparrow$&\text{LPIPS}$\downarrow$\\
        \hline    
        \rowrule w/o distortion field     &17.09&0.426&0.608
                                          &21.67&0.674&0.319\\ 
        \rowrule w/o time axis            &17.25&0.480&0.458
                                          &21.94&0.738&0.279\\
        \rowrule w/o pose axis            &17.38&0.462&0.469
                                          &21.81&0.733&0.268\\
        \rowrule w/o pose optimization    &18.96&0.569&0.336
                                          &22.92&0.754&0.217\\
        \rowrule w/o $\mathcal{L}_{lpips}$&20.61&0.646&0.284
                                          &23.69&0.762&0.185\\
        \hline
        \rowrule \rowcolor{gray!30} Ours         
                                        &\textbf{21.56}&\textbf{0.656}&\textbf{0.264}
                                        &\textbf{24.36}&\textbf{0.793}&\textbf{0.170} \\
        \bottomrule[2pt]
    \end{tabular}
    }
\label{tab:ablation}
\vspace{-3mm}
\end{table}

==> tab/table1.tex <==
\begin{center}    
    \begin{tabular}{ll}
        \multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
        \\ \hline \\
        Dendrite         &Input terminal \\
        Axon             &Output terminal \\
        Soma             &Cell body (contains cell nucleus) \\
    \end{tabular}    
\end{center}

